LAMP: Learn A Motion Pattern for Few-Shot-Based Video Generation

With the impressive progress in diffusion-based text-to-image generation, extending such powerful generative ability to text-to-video raises enormous attention. Existing methods either require large-scale text-video pairs and a large number of training resources or learn motions that are precisely aligned with template videos. It is non-trivial to balance a trade-off between the degree of generation freedom and the resource costs for video generation. In our study, we present a few-shot-based tuning framework, LAMP, which enables text-to-image diffusion model Learn A specific Motion Pattern with 8~16 videos on a single GPU. Specifically, we design a first-frame-conditioned pipeline that uses an off-the-shelf text-to-image model for content generation so that our tuned video diffusion model mainly focuses on motion learning. The well-developed text-to-image techniques can provide visually pleasing and diverse content as generation conditions, which highly improves video quality and generation freedom. To capture the features of temporal dimension, we expand the pretrained 2D convolution layers of the T2I model to our novel temporal-spatial motion learning layers and modify the attention blocks to the temporal level. Additionally, we develop an effective inference trick, shared-noise sampling, which can improve the stability of videos with computational costs. Our method can also be flexibly applied to other tasks, e.g. real-world image animation and video editing. Extensive experiments demonstrate that LAMP can effectively learn the motion pattern on limited data and generate high-quality videos. The code and models are available at https://rq-wu.github.io/projects/LAMP.

==> sec/0_abstract.tex <==
\begin{abstract}
With the impressive progress in diffusion-based text-to-image generation,  extending such powerful generative ability to text-to-video raises enormous attention.
%
Existing methods either require large-scale text-video pairs and a large number of training resources or learn motions that are precisely aligned with template videos.
%
It is non-trivial to balance a trade-off between the degree of generation freedom and the resource costs for video generation.
%
In our study, we present a few-shot-based tuning framework, \textbf{\methodname},
which enables text-to-image diffusion model \textbf{L}earn \textbf{A} specific \textbf{M}otion \textbf{P}attern with 8 $\sim$16 videos on a single GPU.
%
Specifically, we design a first-frame-conditioned pipeline that uses an off-the-shelf text-to-image model for content generation so that our tuned video diffusion model mainly focuses on motion learning.
%
% Under the strong conditions provided by the first frame, the pipeline complements the lack of content diversity with limited data and highly improves the video quality.
The well-developed text-to-image techniques can provide visually pleasing and diverse content as generation conditions, which highly improves video quality and generation freedom.
%
To capture the features of temporal dimension, we expand the pre-trained 2D convolution layers of the T2I model to our novel temporal-spatial motion learning layers and modify the attention blocks to the temporal level.
%\lichongyi{we may need to explain why  2D Conv layers are used, say its function here, and what is `original'. You mean commonly used in diffusion models?} \lichongyi{Please give some details on how to modify.}
Additionally, we develop an effective inference trick, shared-noise sampling, which can improve the stability of videos with computational costs.
%\lichongyi{you may want to say without computational costs?}.
% \lichongyi{If we use interesting, we may need to give some details on why it is interesting.} 
Our method can also be flexibly applied to other tasks, e.g. real-world image animation and video editing.
%
Extensive experiments demonstrate that \methodname~can effectively learn the motion pattern on limited data and generate high-quality videos.
%
The code and models will be released.

% With the impressive progress in text-to-image generation achieved by diffusion-based models, 
% how to extend the powerful generative ability to text-to-video raises enormous attention.
% %
% However, the existing methods either require large-scale text-video pairs and a large amount of training resources or learn motions that are precisely aligned with template videos, which is also known as video editing.
% %
% A trade-off between the degree of generation freedom and the resource cost becomes a challenge to overcome.
% %
% In our work, we present a few-shot-based tuning framework, \textbf{\methodname},
% which can make a text-to-image diffusion model \textbf{L}earn \textbf{A} specific \textbf{M}otion \textbf{P}attern with 8 $\sim$16 videos and a single GPU.
% %
% Specifically, we design a first-frame-conditioned training pipeline that uses an off-the-shelf text-to-image model for content generation and makes our tuned video diffusion model focus on motion learning.
% %
% % Under the strong conditions provided by the first frame, the pipeline complements the lack of content diversity with limited data and highly improves the video quality.
% The well-developed text-to-image techniques can provide visual-pleased and diverse content as generation conditions, which highly improves video quality and generation freedom.
% %
% Moreover, it makes our model can be flexibly applied to other tasks, \eg real-world image animation and video editing.
% %
% To enable the model to capture the features of temporal dimension, we expand the original 2D convolution layers to our novel temporal-spatial motion learning layers and modify the attention blocks.
% %
% Additionally, we develop an interesting inference trick, shared-noise sampling, which can improve the stability of videos freely.
% %
% Extensive experiments demonstrate that \methodname~can effectively learn the motion pattern on limited data and generate high-quality videos.
% %
% The code and models will be released.
\end{abstract}
